Branched coverings of the 2-sphere

Thurston obtained a combinatorial characterization for generic branched self-coverings that preserve the orientation of the oriented 2-sphere by associating a planar graph to them [arXiv:1502.04760]. In this work, the Thurston result is generalized to any branched covering of the oriented 2-sphere. To achieve that the notion of local balance introduced by Thurston is generalized. As an application, a new proof for a Theorem of Eremenko-Gabrielov-Mukhin-Tarasov-Varchenko [MR1888795], [MR2552110] is obtained. This theorem corresponded to a special case of the B. \& M. Shapiro conjecture. In this case, it refers to generic rational functions stating that a generic rational function $ R : \mathbb{C}\mathbb{P}^1 \rightarrow \mathbb{C}\mathbb{P}^1$ with only real critical points can be transformed by post-composition with an automorphism of $\mathbb{C}\mathbb{P}^1$ into a quotient of polynomials with real coefficients. Operations against balanced graphs are introduced.

==> Makefile <==
# 
# makefile para a compilação do documento
#
# Sáb Jun 23 21:13:37 BRT 2007
#

BASE_NAME = tese-exemplo

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex 
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<
	$(PDFLATEX) $<

$(BASE_NAME).ps: $(BASE_NAME).tex 
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(LATEX) $< 
	$(LATEX) $<
	$(LATEX) $<
	
clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 


==> cap-conclusoes.tex <==
%% ------------------------------------------------------------------------- %%
\chapter[Closing remarks and perspectives]{\rule[0ex]{16.5cm}{0.2cm}\vspace{-23pt}
\rule[0ex]{16.5cm}{0.05cm}\\Closing remarks and perspectives}
\label{cap:conclusoes}

%\footnote{Exemplo de referência para página
%Web: \url{www.vision.ime.usp.br/~jmena/stuff/tese-exemplo}}.


\begin{itemize}
\item[$\bullet$]{establish a good correspondence between the balanced graphs(our combinatorial model) and the isomorphism classes of branched covers of $\CPu$;
\begin{itemize}
\item[$\star$]{about the realizability(in genus $0$): we know that the global balancy condition correspond to the passport to enjoy the \emph{Riemann-Hurwitz} formula. So can we encode the local balance condition into condition(s) over a passport?}
\end{itemize}}
\item[$\bullet$]{to count such graphs(using topological recursion, matrix integrals and some more standard combinatorial techniques)P.S.: seems to exist interesting possible connection with the theory of quantum cohomology, Gromov-Witten invariants and 2D TQFT;
\begin{itemize}
\item[$\star$ $\star$]{to establish the generating series for counting of the balanced graphs and shows if it satisfies some integrability condition as: KP-hierarchy,KdV hierarchy, Virasoro constraints, Toda equations, an evolution equation, like Hurwitz numbers does.}
\end{itemize}}
\item[$\bullet$]{to describe the bifurcation of the pullback graphs(=balanced graphs);}
\item[$\bullet$]{to explore the relation between the category of topologycal branched coverings and its subcategory of holomorphic branched coverings(rational functions-recall the Thurston's classification theorem of rational functions);}
\item[$\bullet$]{to scrutiny the relation between the moduli spaces of selfcovers of $\s^2$(for those two types of isomorphims-pre and post composition with appropriate morphisms) and the teichmüller spaces of marked spheres.}
\end{itemize}

Another reason is the possibility of the occurrence of a \emph{Reconstrution Principle}, that is, the possibility of the validity of the conjectural fact that any balanced graph can be obtained by the more simplest ones in genus $0$ and $1$ through concatenation of operations. This operations leads to the class of \emph{Balanced Graphs} the structure of a \emph{Monoidal Groupoid}.  And this brings us to perscrute the relation with 2D TQFT. Is expected that, as in \cite{ss} , this operation may produce relations into the algebra of the generating series for the counting of the balanced graphs and in the topological recursion for them.
Anoter rason is to use these approach to the branched selfcoverings to achieve the combinatorial proof asked by Lisa Goldberg in \cite[{PROBLEM}, at page $132$]{Gold:91} to the counting problem of equivalence classes of generic rational functions of $\CPu$ for prescribed critical points in general position. 

==> cap-introducao.tex <==
%% ------------------------------------------------------------------------- %%
\chapter{Introduction}
\label{cap:intro}



% \emph{Thesis are random access. Do NOT feel obliged to read a thesis from beginning to end.}



%% ------------------------------------------------------------------------- %%
%\section{Outline}\label{sec:outl}

Este trabalho teve inicio com a tarefa dada por \emph{Sylvain Bonnot} de desenvolver um programa no software \href{https://www.wolfram.com/mathematica/}{Mathematica} que desenhasse para uma função racional com coeficientes reais de grau $3$ da forma $\phi_a:z\mapsto \dfrac{az^3 +(1-2a)z^2}{(2-a)z-1}$ a pré-imagem da reta real por esta função. Os pontos críticos $\phi_a$ estão contidos em $\rr$, a saber são eles: $0$, $1$, $\infty$ e $c(a)=\dfrac{2a-1}{a(2-a)}$. Para cada uma destas funções %como descrita anteriormente 
a imagem inversa da reta real produz um grafo celularmente mergulhado em $\cc$, isto é, uma decomposição celular de $\cc$. O interesse de \emph{Sylvain Bonnot} era %A tarefa que decorre da primeira estabelecida era 
descrever como estes grafos variam a medida que variamos o ponto crítico $c(a)$. Isto foi feito e é apresentado no Capítulo $\ref{cap-04}.$

O intuito central da pesquisa apresentada nesta tese consiste em determinar invariantes de caráter combinatórios que possam caracterizar funções racionais considerando-se a sua configuração crítica. Consistindo, portanto em uma teoria dual a aquela iniciada por Hurwitz que estuda os recobrimentos ramificados da esfera bidimencional $\s^2$ levando em consideração os valores críticos.

A família de funções $\phi_a$ foi apresentada por \emph{Sylvain Bonnot} através de uma postagem de \href{http://www.math.hawaii.edu/~xander/index.html}{Xander Faber} no site de perguntas \& respostas de \emph{Matemática}, \href{https://mathoverflow.net/}{Mathoverflow}. Como o título da postagem presume, \href{https://mathoverflow.net/questions/102506/determining-rational-functions-by-their-critical-points?rq=1}{Determining rational functions by their critical points}, \emph{Xander Faber} chama a atenção para o problema da determinação das funções racionais a partir de seus pontos críticos.

Cumprindo o desígnio enunciado acima % nos propomos a apresentar uma
propomos uma descrição combinatória dos recobrimentos ramificados da esfera bidimensional $\s^2$ através de um grafo  %que preservam orientação 
com respeito a sua configuração crítica. A configuração crítica de um recobrimento ramificado consiste na descrição de seus pontos críticos, suas multiplicidades e seus agrupamentos de acordo com suas imagens. Estas informações são dadas através do passaporte(marcado), que é uma lista de partições do grau do recobrimento juntamente com a sequência de pontos críticos em $\s^2$.

A noção de equivalência adequada para a classificação dos recobrimentos ramificados segundo a sua configuração crítica é a que os identifica via póscomposição com homeomorfismos de $\s^2$ que preservam a orientação. Tal equivalência é considerada adequada devido ao fato de preservar a configuração crítica.

No contexto estrito das funções racionais da \emph{esfera de Riemann} $\CPu$ a equivalência considerada é aquela que identifica as funções racionais por póscomposição com automorfismos de $\CPu$, isto é, por póscomposição com \emph{Transformações de Möebius}. 

Um problema natural que surge é aquele sobre a contagem das classes de equivalências para uma configuração prescrita. Alguns resultados para este problema são conhecidos como será descrito mais abaixo.

Este trabalho considera o problema de estabelecer de forma combinatória a contagem das classes de equivalências para uma configuração crítica dada.% um passaporte e os pontos críticos. % Ou o mais próximo disso possível.

Para tanto associaremos a um recobrimento crítico um objeto combinatório, um grafo (celularmente) mergulhado em $\s^2$, isto é, uma decomposição celular de $\s^2$. 

Estes grafos foram introduzidos por \emph{W. Thurston} ao perseguir o problema de determinar qual a forma de uma função racional da linha projetiva complexa $\CPu$. Este problema foi apresentado por Thurston em sua pagina no website de perguntas \& respotas de matemática, \emph{Mathoverflow} << \href{https://mathoverflow.net/questions/38274/what-are-the-shapes-of-rational-functions}{what-are-the-shapes-of-rational-functions}>>, veja também \cite{STL:15}.

O problema de contar tais classes de equivalências de funções racionais de $\CPu$ foi considerado anteriormente por \emph{Eisenbud} \& \emph{Harris} em \cite{EiH:83} e por \emph{Lisa Goldberg} em \cite{Gold:91}. \emph{Goldberg} estabeleceu que fixando o grau $d>0$ e impondo que as funções racionais possuam $2d-2$ pontos críticos com multiplicidade $2$, então para uma lista de $2d-2$ pontos em posição geral em $\CPu$ existem no máximo
\[\rho(d):=\frac{1}{d}{2d-2\choose d-1}\] 
classes de equivalências. 

\begin{comment}(\textcolor{red}{melhorar isto, o problema é considerado em \cite{EiH:83} antes de \cite{Gold:91}})O problema de contar tais classes de equivalências de funções racionais de $\CPu$ foi primeiramente considerado por \emph{Lisa Goldberg} em \cite{Gold:91}. \emph{Goldberg} estabeleceu que fixando o grau $d>0$ e impondo que as funções racionais possuem $2d-2$ pontos críticos com multiplicidade $2$, então para uma lista de $2d-2$ pontos em posição geral em $\CPu$ existem %no máximo
\[\rho(d):=\frac{1}{d}{2d-2\choose d-1}\] 
classes de equivalências.\end{comment}

Este resultado foi estabelecido usando-se da \emph{Geometria Algébrica}, mais precisamente traduzindo-o em um problema de \emph{Schubert} para subespaços bi-dimencionais de Grassmanianas.
%do \emph{Cálculo de Schubert}. 

O inteiro $\rho (d)$ é denominado por $d$-\emph{ésimo número de Catalan}. Estes números são altamente presentes e recorrentes na \emph{Matemática Discreta}, possuindo um enorme número de interpretações combinatórias. Além disto, \emph{os números de Catalan} costumam
se manifestar em diversas áreas fora da \emph{Matemática Discreta} sem que haja uma evidente razão combinatória pra tal aparição.
%aparecer como caso particulares de formulas mais gerais,
Por exemplo, %no problema de contagem de (non)standard Young Tableaux na \emph{Análise Combinatória}, ou 
no problema de determinar o grau de aplicações ou dimensão de variedades algébricas na \emph{teoria de interseção} \cite{GH:94} e \emph{Cálculo de Schubert} \cite{GH:94} para Grassmanianas.
%, que, a priori, não são problemas da \emph{Matemática Discreta}.

Uma solução completa com a obtenção de uma fórmula genérica para este problema foi dada por I. Scherbak em \cite{Scherbak:02}. Tal resultado foi estabelecido através da combinação do \emph{Cálculo de Schubert, Teoria de Representação, Equações Diferenciais Fuchsianas e Teoria das Equações de KZ}.

Fazendo uso da Teoria das Séries Lineares Limite desenvolvida por  \emph{Eisenbud} \& \emph{Harris} em \cite{EiH:86}, B. Osserman em \cite{Oss:03} estabeleceu a contagem para o caso mais geral de recobrimentos ramificados da esfera de gênero positivo.

Eremenko e Gabrielov em \cite{MR1888795} ao provarem o caso mais simples da conjectura de \emph{B} \& \emph{M Shapiro} mostraram que o número de classes de equivalências de funções racionais de grau $d$ com $2d-2$ pontos críticos prescritos contidos em $\RPu$ é pelo menos $\rho(d).$ 
%se os $2d-2$ pontos críticos de uma função racional de grau $d$ são todos reais, isto é, estão contidos em $\RPu$, então existem pelo menos $\rho(d)$ classes de equivalências de funções racionais de grau $d$ que possuem estes pontos como pontos críticos.
A conjectura de \emph{B} \& \emph{M Shapiro}, hoje um teorema devido aos matemáticos E. Mukhin, V. Tarasov e  A. Varchenko \cite{MR2552110}, afirma que se o \emph{Determinante Wronskiano} de uma lista de polinômios de grau $d$ com coeficientes complexos, $f_1(z), f_2(z), \cdots ,f_d(z)\in\C [z]$, só possue zeros reais, então o subespaço vetorial $\langle f_1(z), f_2(z), \cdots ,\\ f_d(z)\rangle_{\C}\subset \C [z]$ possue uma base em $\R [z]$. Em \cite{MR1888795}, Eremenko e Gabrielov introduziram uma decomposição celular da \emph{esfera de Riemann} $\CPu$, a qual chamaram de ``net''. Eles utilizam esta decomposição celular da esfera para construir o número eperado de classes de funções racionais reais. Estes grafos celulares são exemplos particulares dos \emph{grafos balanceados} introduzidos por \emph{Thurston}\;\cite{STL:15}. %no entanto, eles não se atentam para este fato, isto é, para o potencial de tais grafos como representantes de recobrimentos ramificados da esfera $\s^2$. 

Thurston \cite{STL:15} estabeleceu uma completa caracterização combinatória dos autorecobrimentos ramificados genéricos da esfera bidimensional $\s^2$. Um recobrimento ramificado de grau $d$, $\s^2\rightarrow\s^2$, é dito genérico quando possue o número máximo de pontos críticos que é $2d-2$(ou equivalentemente, quando todos os seus pontos cŕiticos possuem multiplicidade $2$).

\begin{thm}[\cite{STL:15}]
 An oriented planar graph $\Gamma$ with $2d-2$ vertices of valence $4$ is equal to $f^{-1}(\Sigma)$ for some degree $d$ branched cover $f:\s^2 \rightarrow\s^2$ and some $\Sigma$ if and only if
 \begin{itemize}
 \item[1]{every face of $\Gamma$ is a Jordan domain (in particular $\Gamma$ is connected);}
\item[2]{(global balance) for any alternating white-blue coloring of the faces of $\Gamma$, there are $d$ white faces, and there are d blue faces, and}
\item[3]{(local balance) for any oriented simple closed curve in $\Gamma$ that is bordered by blue faces on the left and white on the right (except at the corners), there are strictly more blue faces than white faces on the left side of $\Gamma$.}
\end{itemize}
\end{thm} See Chapter $\ref{cap-03}$ for definitions.%\ref{sect-thurstonthm}





\paragraph{o que temos feito}
\begin{itemize}
\item{generalização de um teorema de Thurston;}
\item{prova de um caso da conjectura de B \& M Shapiro;}
\item{estudo as funções racionais cúbica genéricas-grafo pullback;}
\end{itemize} 

\begin{comment}
\section{Como este trabalho começou:}

Este trabalho teve inicio com a tarefa dada por \emph{Sylvain Bonnot} de desenvolver um programa no software \href{https://www.wolfram.com/mathematica/}{Mathematica} que desenhasse para uma função racional com coeficientes reais de grau $3$ da forma $\phi_a:z\mapsto \dfrac{az^3 +(1-2a)z^2}{(2-a)z-1}$ a pré-imagem da reta real por esta função. Os pontos críticos $\phi_a$ estão contidos em $\rr$, a saber são eles: $0$, $1$, $\infty$ e $c(a)=\dfrac{2a-1}{a(2-a)}$. Para cada uma destas funções %como descrita anteriormente 
a imagem inversa da reta real produz um grafo celularmente mergulhado em $\cc$, isto é, uma decomposição celular de $\cc$. O interesse de \emph{Sylvain Bonnot} era %A tarefa que decorre da primeira estabelecida era 
descrever como estes grafos variam a medida que variamos o ponto crítico $c(a)$. Isto foi feito e é apresentado no Capítulo $\ref{cap-04}.$

O intuito central da pesquisa apresentada nesta tese consiste em determinar invariantes de caráter combinatórios que podessem caracterizar funções racionais considerando-se a sua configuração crítica. Consistindo portanto em uma teoria dual a aquela iniciada por Hurwitz que leva em consideração os valores críticos.

A família de funções $\phi_a$ foi apresentada por \emph{Sylvain Bonnot} através de uma postagem de \href{http://www.math.hawaii.edu/~xander/index.html}{Xander Faber} no site de perguntas \& respostas de \emph{Matemática}, \href{https://mathoverflow.net/}{Mathoverflow}. Como o título da postagem presume, \href{https://mathoverflow.net/questions/102506/determining-rational-functions-by-their-critical-points?rq=1}{Determining rational functions by their critical points}, \emph{Xander Faber} chama a atenção para o problema da determinação das funções racionais a partir de seus pontos críticos.

\end{comment}




%\footnote{Nota de rodapé (não abuse).}
%\index{genoma!projetos}% index permite acrescentar um item no indice remissivo

 
\begin{comment}
%% ------------------------------------------------------------------------- %%
\section{Goals}
\label{sec:obj}

\begin{itemize}
\item[$\bullet$]{establish a good correspondence between the balanced graphs(our combinatorial model) and the isomorphism classes of branched covers of $\CPu$;
\begin{itemize}
\item[$\star$]{about the realizability(in genus $0$): we know that the global balancy condition correspond to the passport to enjoy the \emph{Riemann-Hurwitz} formula. So can we encode the local balancy condition into condition(s) over a passport?}
\end{itemize}}
\item[$\bullet$]{to count such graphs(using topological recursion, matrix integrals and some more standard combinatorial techniques)P.S.: seems to exist interesting possible connection with the theory of quantum cohomology, Gromov-Witten invariants and 2D TQFT;
\begin{itemize}
\item[$\star$ $\star$]{to establish the generating series for counting of the balanceds graphs and shows if it satisfies some integrability condition as: KP-hierarchy,KdV hierarchy, Virasoro constraints, Toda equations, an evolution equation, like Hurwitz numbers does.}
\end{itemize}}
\item[$\bullet$]{to describe the bifurcation of the pullback graphs(=balanced graphs);}
\item[$\bullet$]{to explore the relation between the category of topologycal branched coverings and its subcategory of holomorphic branched coverings(rational functions-recall the Thurston's classification theorem of rational functions);}
\item[$\bullet$]{to scrutiny the relation between the moduli spaces of selfcovers of $\s^2$(for those two types of isomorphims-pre and post composition with appropriate morphisms) and the teichmüller spaces of marked spheres.}
\end{itemize}

%% ------------------------------------------------------------------------- %%
\section{What is new}
\label{sec:contr}
\end{comment}

%% ------------------------------------------------------------------------- 


